Two-Player Zero-Sum Hybrid Games

In this paper, we formulate a two-player zero-sum game under dynamic constraints defined by hybrid dynamical equations. The game consists of a min-max problem involving a cost functional that depends on the actions and resulting solutions to the hybrid system, defined as functions of hybrid time and, hence, can flow or jump. A terminal set conveniently defined allows to recast both finite and infinite horizon problems. We present sufficient conditions given in terms of Hamilton-Jacobi-Bellman-Isaacs-like equations to guarantee to attain a solution to the game. It is shown that when the players select the optimal strategy, the value function can be evaluated without computing solutions to the hybrid system. Under additional conditions, we show that the optimal state-feedback laws render a set of interest asymptotically stable for the resulting hybrid closed-loop system. Applications of these games, presented here as robust control problems, include disturbance rejection and security problems.

==> macros/macrosFF.tex <==
% List of macros that are not in macrosbook.tex and come from rgsMacros.sty 
%\newcommand{\figurename}{Fig.}
\newcommand*{\QEDB}{\hfill\ensuremath{\square}}%
\newcommand{\SH}{\mathcal{S}_{\mathcal{H}_0}}
\newcommand{\range}{\operatorname{rge}}
%\newcommand{\sat}{\operatorname{sat}}
\newcommand{\ess}{\operatorname{ess.}}
\newcommand{\thetatilde}{\tilde{\theta}}
\newcommand{\GtES}{G$_t$ES}
%\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand\ceil[1]{\lceil#1\rceil}
\newcommand{\limsupdomo}{\limsup_{\substack{(t, j)\in\dom\phi_0\\(t, j)\rightarrow\sup\dom\phi_0}}}
\newcommand{\limsupdom}{\limsup_{\substack{(t, j)\in\dom\phi\\(t, j)\rightarrow\sup\dom\phi}}}
\newcommand{\limdom}{\lim_{\substack{(t, j)\in\dom\phi\\(t, j)\rightarrow\sup\dom\phi}}}
\newcommand{\tl}{t\mbox{-}\mathcal{L}_2}
%\newcommand{\A}{\mathcal{A}}
\newcommand{\SHO}{\mathcal{S}_{\mathcal{H}_0}}
%\newcommand{\dom}{\operatorname{dom}}
\newcommand{\Sign}{\operatorname{sign}}
\newcommand{\Id}{I}
\newcommand*{\tr}{^{\mkern-1.5mu\mathsf{T}}}
\newcommand*{\mtr}{^{\mkern-1.5mu\mathsf{-T}}}
\newcommand{\minimize}{\operatorname{minimize}}
\newcommand{\Tr}{\operatorname{trace}}
\newcommand{\Co}{\operatorname{Co}}
\newcommand{\He}{\operatorname{He}}
\newcommand{\Diag}{\operatorname{diag}}
\newcommand{\Int}{\operatorname{int}}
\newcommand{\spec}{\operatorname{spec}}
\newcommand{\Spn}{\mathbb{S}^n_{+}}
\newcommand{\Sn}{\mathbb{S}^n}
\newcommand{\Skewn}{\mathbb{A}^n}
\newcommand{\Spnz}{\mathcal{S}^{n_z}_{+}}
\newcommand{\Spny}{\mathcal{S}^{n_y}_{+}}
\newcommand{\CUD}{\overline{C}\cup D}
\newcommand{\0}{{0}}
\newcommand{\eg}{{\itshape e.g.}}
\newcommand{\Ho}{\mathcal{H}_0}
\newcommand{\ie}{{i.e.}}
\newcommand{\1}{{\bf 1}}
\newcommand{\rk}{{\bf rk}}
\newcommand{\Card}{{\mathcal{C}}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\ep}{{\varepsilon}}
\renewcommand\Im{\operatorname{\mathfrak{Im}}}
\renewcommand\Re{\operatorname{\mathfrak{Re}}}

==> macros/macrosPuP.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  THEOREMS AND ENVIRONMENTS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\newtheorem{nntheorem}{\bf Theorem}[chapter]
%\newtheorem{nnlemma}[nntheorem]{\bf Lemma}
%\newtheorem{nndefinition}[nntheorem]{\bf Definition}
%\newtheorem{nncorollary}[nntheorem]{\bf Corollary}
%\newtheorem{nnproposition}[nntheorem]{\bf Proposition}
%\newtheorem{nnassumption}[nntheorem]{\bf Assumption}
%\newtheorem{nexample}[nntheorem]{\bf Example}
%\newtheorem{nnremark}[nntheorem]{\bf Remark}
%\newtheorem{nnproblem}[nntheorem]{\bf Exercise}

% FOR PUP
%\renewenvironment{theorem}[1]
%{\begin{nntheorem}{\rm\textrm{#1}}\sl}
%{\end{nntheorem}}
%
%% FOR PUP
%\renewenvironment{proposition}[1]
%{\begin{nnproposition}{\rm\textrm{(#1)}}\sl}
%{\end{nnproposition}}
%
%% FOR PUP
%\renewenvironment{lemma}[1]
%{\begin{nnlemma}{\rm\textrm{#1}}\sl}
%{\end{nnlemma}}
%
%\renewenvironment{corollary}[1]
%{\begin{nncorollary}{\rm\textrm{#1}}\sl}
%{\end{nncorollary}}
%
%% FOR PUP
%\renewenvironment{definition}[1]
%{\begin{nndefinition}{\rm\textrm{#1}}\sl}
%{\end{nndefinition}}
%
%
%\newenvironment{assumption}[1]
%{\begin{nnassumption}{\rm\textrm{(#1)}}\sl}
%{\end{nnassumption}}

%\newenvironment{assumption}[1]
%{\begin{nnassumption}{\rm\textrm{#1}}\sl}
%{\end{nnassumption}}

%
%\renewenvironment{example}[1]
%{\begin{nexample}{\rm\textrm{#1}}\rm}
%{\end{nexample}}
%
%% FOR PUP
%\renewenvironment{remark}[1]
%{\begin{nnremark}{\rm\textrm{#1}}\sl}
%{\end{nnremark}}

%%\newenvironment{problem}[1]
%%{\begin{nnproblem}{\rm\textrm{(#1)}}\sl}
%%{\end{nnproblem}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\newcommand{\eoe}
%           {\hspace*{\fill}{$\vcenter{\hrule height1pt 
%                     \hbox{\vrule width1pt height3pt 
%            \kern3pt \vrule width1pt} \hrule height1pt}$} }

% FOR PUP
%\renewenvironment{example}[1]
%{\begin{nexample}{\rm\textrm{(#1)}}\rm}{\eoe\end{nexample}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\newcommand{\eop}
%           {\hspace*{\fill}{$\vcenter{\hrule height1pt 
%                     \hbox{\vrule width1pt height5pt 
%            \kern5pt \vrule width1pt} \hrule height1pt}$} }
%
% FOR PUP
%\newenvironment{proof}
%{\par\noindent\textbf{Proof.}}{\eop\smallskip\vskip 3 pt}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  PRETTY OBVIOUS NEWCOMMANDS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
%\newcommand{\ball}{{\mathbb B}}
%\newcommand{\con}{{\mathop{\rm con}\nolimits}}
%\newcommand{\clcon}{{\overline{\con}}}
%\newcommand{\dom}{\mathop{\rm dom}\nolimits}
%\newcommand{\glim}{\mathop{\rm gph\mbox{-}lim}}
%\newcommand{\glimsup}{\mathop{\rm gph\mbox{-}lim\,sup}}
%\newcommand{\gliminf}{\mathop{\rm gph\mbox{-}lim\,inf}}
%\newcommand{\gph}{\mathop{\rm gph}\nolimits}
%\renewcommand{\iint}{\mathop{\rm int}\nolimits}
%\newcommand{\integers}{{\mathbb Z}}
%\newcommand{\iti}{{i\to\infty}}
%\newcommand{\kti}{{k\to\infty}}
%\newcommand{\KL}{{{\mathcal{K}\mathcal{L}}}}
%\newcommand{\KLL}{{{\mathcal{K}\mathcal{L}\mathcal{L}}}}
%\newcommand{\naturals}{{\mathbb N}}
%\newcommand{\ox}{{\bar{x}}}
%\newcommand{\reals}{{\mathbb R}}
%\renewcommand{\Re}{{\mathbb R}}
%\newcommand{\realsplus}{{\reals_{\geq 0}}}
%\newcommand{\realspplus}{{\reals_{>0}}}
%\newcommand{\rge}{\mathop{\rm rge}\nolimits}
%\newcommand{\rge}{\mathop{\rm rge}}      
%\newcommand{\rge}{{\mathop{\rm rge}\nolimits}}
%\newcommand{\tto}{\;{\lower 1pt \hbox{$\rightarrow$}}\kern -10pt
%           \hbox{\raise 2pt \hbox{$\rightarrow$}}\;}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  NEWCOMMANDS TO ARGUE ABOUT
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% compact attractor
\newcommand{\A}{\mathcal{A}}
%% a homogeneous ``ball''
%\newcommand{\B}{\mathcal{B}}
%% basin of attraction of a compact attractor
\newcommand{\BA}{\mathcal{B}_\A}
\newcommand{\BAone}{\mathcal{B}_{\A_{1}}}
\newcommand{\BAtwo}{\mathcal{B}_{\A_{2}}}
%% conical approximation symbol
\newcommand{\CA}{\mathcal{CA}}
%% class-K
\newcommand{\classK}{{\mathcal{K}}}
%% class-K function
\newcommand{\classKfunction}{{\alpha}}
%% class-K function lower
\newcommand{\classKfunctionlower}{{\underline{\classKfunction}}}
%% class-K function upper
\newcommand{\classKfunctionupper}{{\overline{\classKfunction}}}
%% class-Kinfty
%\newcommand{\classKinfty}{{\mathcal{K}_\infty}}
%% generic measuement error
\newcommand{\e}{e}
%% global pre asymptotic stability abbreviation
\newcommand{\GpAS}{{GpAS}}
%% a superscript indicating homogeneous things
\newcommand{\homo}{h}
%% hybrid system
\newcommand{\HS}{\mathcal{H}}
%% hybrid system with data
\newcommand{\HSdata}{\HS=(C,F,D,G)}
%% hybrid system data only
\newcommand{\data}{(C,F,D,G)}
%% hybrid system with data (lower case)
\newcommand{\datal}{(C,f,D,g)}
%% hybrid system regularized data only
\newcommand{\regdata}{(\reg{C},\reg{F},\reg{D},\reg{G})}
%% size of a homogeneous perturbation
\newcommand{\homopert}{\eta}
%% hybrid system with measurement error
\newcommand{\HSe}{{\HS_e}}
%% hybrid system, regularized
\newcommand{\HSreg}{{\reg{\HS}}}
%% generic hybrid time domain
\newcommand{\htd}{E}
%% indicator of A 
\newcommand{\indi}{\omega}
%% generic compact set
\newcommand{\K}{K}
%% class KL
\newcommand{\classKL}{{\mathcal{K}\mathcal{L}}}
%% generic KL function
\newcommand{\kl}{\beta}
\newcommand{\classKLfunction}{\beta}
%% length of a hybrid time domain
\newcommand{\length}{\mathop{\rm length}\nolimits}
%% generic set valued mapping
\newcommand{\map}{M}
%% state space
\renewcommand{\O}{O}
%% pre asymptotic stability abbreviation
\newcommand{\pAS}{{pAS}}
%% pre basin of attraction 
\newcommand{\preBA}{{\BA^p}}
\newcommand{\preBAone}{{\BAone^p}}
\newcommand{\preBAtwo}{{\BAtwo^p}}
%% admissible radius of perturbation
\newcommand{\rad}{\rho}
%% reachable set
%\newcommand{\reach}{\mathcal{R}}
%% regularization of C D F G
\newcommand{\reg}[1]{{\widehat{#1}}}
%% saturation function
\newcommand{\sat}{{sat}}
%% sequence, for example \seq{x}{i} produces \{x_i\}_{i=0}^\infty
\newcommand{\seq}[2]{{\{#1_{#2}\}_{#2=1}^\infty}}
%% subsequence, for example \seq{x}{i}{k} produces \{x_{i_k}\}_{i=0}^\infty
\newcommand{\subseq}[3]{{\{#1_{#2_{#3}}\}_{#3=1}^\infty}}
%% generic set
\newcommand{\set}{S}
%% solution to a hybrid system or just a hybrid arc
\newcommand{\sol}{\phi}
%% alternative solution to a hybrid system or just a hybrid arc
\newcommand{\sola}{\psi}
%% derivative of alternative solution to a hybrid system or just a hybrid arc
\newcommand{\soladot}{\dot{\sola}}
%% difference of alternative solution to a hybrid system of just a hybrid arc
\newcommand{\solaplus}{{\sola^+}}
%% solution to a hybrid closed-loop system (control)
\newcommand{\solcl}{\zeta}
%%
\newcommand{\solcldot}{\dot{\zeta}}
%%
\newcommand{\solclplus}{\zeta^+}
%% initial point for solution to a hybrid system 
\newcommand{\solinit}{\xi}
%% set of maximal solutions to a hybrid system 
\newcommand{\So}{{\mathcal{S}}}
%% set of maximal solutions to a hybrid system \HS
\newcommand{\Sol}{{\mathcal{S}_\HS}}
%% continuous time arc
\newcommand{\solc}{z}
%%
\newcommand{\solcdot}{{\dot{\solc}}}
%%
\newcommand{\soldot}{{\dot{\sol}}}
%% discrete time arc
\newcommand{\sold}{z}
%%
\newcommand{\soldplus}{\sold^+}
%%
\newcommand{\solplus}{{\sol^+}}
%% symbol for switching system
\renewcommand{\SS}{\Sigma}
%\renewcommand{\SS}{\mathcal{S}}
%% supremum in time of a hybrid time domain
\newcommand{\supt}{{\sup\nolimits_t}} 
%% supremum in jumps of a hybrid time domain
\newcommand{\supj}{{\sup\nolimits_j}}
%% generic open set 
\newcommand{\U}{\mathcal{U}}
%% text referring to the type of document is being compiled
\newcommand{\book}{book}
%% well posed
\newcommand{\wellposed}{nominally well-posed}
%% well posed
\newcommand{\Wellposed}{Nominally well-posed}
%% very well posed
\newcommand{\verywellposed}{well-posed}
%% very well posed
\newcommand{\Verywellposed}{Well-posed}
% set
% \newcommand{\bigbrace}[1]{\left\{#1\right\}}
% \newcommand{\set}[2]{\bigbrace{#1\ \left| \ #2 \right.}}
% \newcommand{\setsmall}[2]{\{#1\ | \ #2 \}}

%% j-th interval for continuous time t
\newcommand{\intj}{I^j}
%% J-th interval for continuous time t
\newcommand{\intJ}{I^J}
%% 0-th interval for continuous time t
\newcommand{\intzero}{I^0}
%% shorthand for varepsilon
\newcommand{\eps}{\varepsilon}
%% shorthand for \overline
\newcommand{\ol}[1]{\overline{#1}}
%% matrix 
\newcommand{\matt}[1]{\begin{bmatrix}#1\end{bmatrix}} 
%% set definition
\newcommand{\bigbrace}[1]{\left\{#1\right\}}
\newcommand{\defset}[2]{\bigbrace{#1\, : \, #2 }}
% sign function
\newcommand{\sign}{{\mathop{\rm sign}\nolimits}}
% floor function
\newcommand{\floor}{{\mathop{\rm floor}\nolimits}}
%
\newcommand{\HBC}{hybrid basic conditions}
% vertical vector
\newcommand{\vect}[1]{{\left(\begin{matrix}#1\end{matrix}\right)}}
% CT plants data
%\newcommand{\fp}{\widetilde{f}}


%% LOCALIZATION
\newcommand{\floc}{f_{loc}}
\newcommand{\gloc}{g_{loc}}
\newcommand{\Cloc}{C_{loc}}
\newcommand{\Dloc}{D_{loc}}


%%% UNIFORM FORMULAS FOR STUFF
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% hybrid system with no name and eight parameters:
%% variable, flow set, \in or =, flow map, jump set, \in or =, jump map
\newcommand{\hybridsystem}[7]
{
\left\{
{
\setlength\extrarowheight{.2cm}
\begin{array}{c@{\ }c@{\ }ccc@{\ }c@{\ }c}
#1 &\in&#2 & \ & \dot{#1} & #3 & #4\left(#1\right) \cr
#1 &\in&#5 & \ & {#1}^+   & #6 & #7\left(#1\right)   \cr
\end{array}
}
\right.
}

%% hybrid system with no name and six parameters:
%% variable, flow set, flow map, jump set, jump map
%% inclusions only
\newcommand{\hybridinclusion}[5]
{
\hybridsystem{#1}{#2}{\in}{#3}{#4}{\in}{#5}
}


%% hybrid system with a name and nine parameters:
%% name, variable, flow set, \in or =, flow map, jump set, \in or =, jump map
\newcommand{\hybridsystemwithname}[8]
{
#1: \qquad 
\hybridsystemn{#2}{#3}{#4}{#5}{#6}{#7}{#8}
}


%% hybrid system with a name and seven parameters:
%% name, variable, flow map, flow set, jump map, jump set
\newcommand{\hybridinclusionwithname}[6]
{
#1: \qquad 
\hybridinclusion{#2}{#3}{#4}{#5}{#6}
}

%% hybrid system with logical modes 
%% discrete variable, continuous variable, flow set, \in or =, flow map, jump set, \in or =, jump map (data with no subscripts)
\newcommand{\hybridsystemQ}[8]
{
\left\{
{
\setlength\extrarowheight{.2cm}
\begin{array}{c@{\ }c@{\ }ccc@{\ }c@{\ }c}
#2 & \in & {#3}_{#1} & \ & \dot{#2}    & #4 & {#5}_{#1}\left(#2\right) \cr
#2 & \in & {#6}_{#1} & \ & {(#1,#2)}^+ & #7 & {#8}_{#1}\left(#2\right)  \cr
\end{array}
}
\right.
}


%% data of a hybrid system, first line C, f or F, second line D, g or G. parameters
%% variable, label for C, formula for C, f or F etc, formula for F, label for D, formula for D, g or G etc, formula for G, 
\newcommand{\definehybridsystem}[9]
{
\setlength\extrarowheight{.2cm}
\begin{array}{r@{\ }c@{\ }lcr@{\ }c@{\ }l}
\displaystyle{#2} & = & \displaystyle{#3} & \qquad &
\displaystyle{#4\left(#1\right)} & = & \displaystyle{#5} \\
\displaystyle{#6} & = & \displaystyle{#7} & \qquad &
\displaystyle{#8\left(#1\right)} & = & \displaystyle{#9}
\end{array}
}


%%% Highlight modifications
\def\startmodif{\color{blue}}
\def\stopmodif{\color{black}\normalcolor}



%%% Comments
%\newcommand{\rafal}[1]{{\noindent \color{red} \tt \small #1}}
%\newcommand{\andy}[1]{{\noindent \color{green} \tt \small #1}}
%\newcommand{\ricardo}[1]{{\noindent \color{blue} \tt \small #1}}
%\def\startmodif{\color{red}}
%\def\stopmodif{\color{black}\normalcolor}
%
%\def\startmodifa{\color{green}}
%\def\stopmodifa{\color{black}\normalcolor}
%
%\def\startmodifaa{\color{black}}
%\def\stopmodifaa{\color{black}\normalcolor}
%
%\def\startmodifr{\color{blue}}
%\def\stopmodifr{\color{black}\normalcolor}
%
%\def\startmodifra{\color{black}}
%\def\stopmodifra{\color{black}\normalcolor}


\newcommand{\Sphere}{\mathbb{S}}

\newcommand{\T}{\mathcal{T}}














==> macros/macrosbook.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  THEOREMS AND ENVIRONMENTS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newtheorem{nntheorem}{ Theorem}[section]
\newtheorem{nnlemma}[nntheorem]{ Lemma}
\newtheorem{nndefinition}[nntheorem]{ Definition}
\newtheorem{nncorollary}[nntheorem]{ Corollary}
\newtheorem{nnconjecture}[nntheorem]{ Conjecture}
\newtheorem{nnproposition}[nntheorem]{ Proposition}
\newtheorem{nnassumption}[nntheorem]{ Assumption}
\newtheorem{nexample}[nntheorem]{ Example}
\newtheorem{nnremark}[nntheorem]{ Remark}\newtheorem{nnapplication}[nntheorem]{ Application}
\newtheorem{nnproblem}[nntheorem]{ Exercise}

\newenvironment{theorem}[1]
{\begin{nntheorem}{\rm\textrm{(#1)}}\sl}
{\end{nntheorem}}

\newenvironment{proposition}[1]
{\begin{nnproposition}{\rm\textrm{(#1)}}\sl}
{\end{nnproposition}}

\newenvironment{lemma}[1]
{\begin{nnlemma}{\rm\textrm{(#1)}}\sl}
{\end{nnlemma}}

\newenvironment{corollary}[1]
{\begin{nncorollary}{\rm\textrm{(#1)}}\sl}
{\end{nncorollary}}

\newenvironment{conjecture}[1]
{\begin{nnconjecture}{\rm\textrm{(#1)}}\sl}
{\end{nnconjecture}}


\newenvironment{definition}[1]
{\begin{nndefinition}{\rm\textrm{
\ifx\hfuzz#1\hfuzz
\else
  (#1)%
\fi
}}\sl}
{\end{nndefinition}}

\newenvironment{assumption}[1]
{\begin{nnassumption}{\rm\textrm{
\ifx\hfuzz#1\hfuzz%%Check if it is empty
%% don't include anything in the name of the result
\else
  (#1)% include the input in the name of the result
\fi
}}\sl}
{\end{nnassumption}}

\newenvironment{application}[1]
{\begin{nnapplication}{\rm\textrm{(#1)}}\sl}
{\end{nnapplication}}

\newenvironment{remark}[1]
{\begin{nnremark}{\rm\textrm{(#1)}}\sl}
{\end{nnremark}}

\newenvironment{problem}[1]
{\begin{nnproblem}{\rm\textrm{(#1)}}\sl}
{\end{nnproblem}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\eoe}
           {\hspace*{\fill}{$\vcenter{\hrule height1pt 
                     \hbox{\vrule width1pt height3pt 
            \kern3pt \vrule width1pt} \hrule height1pt}$} }

\newenvironment{example}[1]
{\begin{nexample}{\rm\textrm{(#1)}}\rm}{\eoe\end{nexample}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\eop}
           {\hspace*{\fill}{$\vcenter{\hrule height1pt 
                     \hbox{\vrule width1pt height5pt 
            \kern5pt \vrule width1pt} \hrule height1pt}$} }

%\newenvironment{proof}
%{\par\noindent\textbf{Proof.}}{\eop\smallskip\vskip 3 pt}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  PRETTY OBVIOUS NEWCOMMANDS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
\newcommand{\ball}{{\mathbb B}}
\newcommand{\con}{{\mathop{\rm con}\nolimits}}
\newcommand{\clcon}{{\overline{\con}}}
\newcommand{\dom}{\mathop{\rm dom}\nolimits}
\newcommand{\glim}{\mathop{\rm gph\mbox{-}lim}}
\newcommand{\glimsup}{\mathop{\rm gph\mbox{-}lim\,sup}}
\newcommand{\gliminf}{\mathop{\rm gph\mbox{-}lim\,inf}}
\newcommand{\gph}{\mathop{\rm gph}\nolimits}
\renewcommand{\iint}{\mathop{\rm int}\nolimits}
\newcommand{\integers}{{\mathbb Z}}
\newcommand{\iti}{{i\to\infty}}
\newcommand{\kti}{{k\to\infty}}
\newcommand{\KL}{{{\mathcal{K}\mathcal{L}}}}
\newcommand{\KLL}{{{\mathcal{K}\mathcal{L}\mathcal{L}}}}
\newcommand{\naturals}{{\mathbb N}}
\newcommand{\ox}{{\bar{x}}}
\newcommand{\reals}{{\mathbb R}}
\renewcommand{\Re}{{\mathbb R}}
\newcommand{\realsplus}{{\reals_{\geq 0}}}
\newcommand{\realspplus}{{\reals_{>0}}}
\newcommand{\rge}{\mathop{\rm rge}\nolimits}
%\newcommand{\rge}{\mathop{\rm rge}}      
%\newcommand{\rge}{{\mathop{\rm rge}\nolimits}}


% \newcommand{\tto}{\;{\lower 1pt \hbox{$\rightarrow$}}\kern -10pt
%            \hbox{\raise 2pt \hbox{$\rightarrow$}}\;}

\newcommand{\tto}{\;{\lower 1pt \hbox{$\rightarrow$}}\kern -12pt
           \hbox{\raise 2pt \hbox{$\rightarrow$}}\;}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  NEWCOMMANDS TO ARGUE ABOUT
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% compact attractor
\newcommand{\A}{\mathcal{A}}
%% basin of attraction of a compact attractor
\newcommand{\BA}{\mathcal{B}_\A}
%% generic measuement error
%\newcommand{\e}{e}
%% hybrid system
\newcommand{\HS}{\mathcal{H}}
%% hybrid DAE system
\newcommand{\Hdae}{\mathcal{H}_{DAE}}
%% hybrid system with data
\newcommand{\HSdata}{\HS=(O,F,C,G,D)}
%% hybrid system data only
\newcommand{\data}{(O,F,C,G,D)}
%% hybrid system with data (lower case)
\newcommand{\datal}{(O,f,C,g,D)}
%% hybrid system regularized data only
\newcommand{\regdata}{(O,\reg{F},\reg{C},\reg{G},\reg{D})}
%% hybrid system with measurement error
\newcommand{\HSe}{{\HS_e}}
%% hybrid system, regularized
\newcommand{\HSreg}{{\reg{\HS}}}
%% generic hybrid time domain
\newcommand{\htd}{E}
%% indicator of A 
\newcommand{\indi}{\omega}
%% generic compact set
\newcommand{\K}{K}
%% generic KL function
\newcommand{\kl}{\gamma}
%% length of a hybrid time domain
\newcommand{\length}{\mathop{\rm length}\nolimits}
%% generic set valued mapping
\newcommand{\map}{M}
%% state space
\renewcommand{\O}{O}
%% pre basin of attraction 
\newcommand{\preBA}{{\BA^p}}
%% admissible radius of perturbation
\newcommand{\rad}{\rho}
%% reachable set
%\newcommand{\reach}{\mathcal{R}}
%% regularization of C D F G
\newcommand{\reg}[1]{{\widehat{#1}}}
%% saturation function
\newcommand{\sat}{{\rm sat}}
%% sequence, for example \seq{x}{i} produces \{x_i\}_{i=0}^\infty
\newcommand{\seq}[2]{{\{#1_{#2}\}_{#2=1}^\infty}}
%% subsequence, for example \seq{x}{i}{k} produces \{x_{i_k}\}_{i=0}^\infty
\newcommand{\subseq}[3]{{\{#1_{#2_{#3}}\}_{#3=1}^\infty}}
%% generic set
\newcommand{\set}{S}
%% solution to a hybrid system or just a hybrid arc
\newcommand{\sol}{\phi}
%% solution to a hybrid closed-loop system (control)
\newcommand{\solcl}{\zeta}
%%
\newcommand{\solcldot}{\dot{\zeta}}
%%
\newcommand{\solclplus}{\zeta^+}
%% initial point for solution to a hybrid system 
\newcommand{\solinit}{\xi}
%% set of maximal solutions to a hybrid system 
\newcommand{\So}{{\mathcal{S}}}
%% set of maximal solutions to a hybrid system \HS
\newcommand{\Sol}{{\mathcal{S}_\HS}}
%% continuous time arc
\newcommand{\solc}{z}
%%
\newcommand{\solcdot}{{\dot{\solc}}}
%%
\newcommand{\soldot}{{\dot{\sol}}}
%% discrete time arc
\newcommand{\sold}{z}
%%
\newcommand{\soldplus}{\sold^+}
%%
\newcommand{\solplus}{{\sol^+}}
%% symbol for switching system
\renewcommand{\SS}{\Sigma}
%\renewcommand{\SS}{\mathcal{S}}
%% supremum in time of a hybrid time domain
\newcommand{\supt}{{\sup\nolimits_t}} 
%% supremum in jumps of a hybrid time domain
\newcommand{\supj}{{\sup\nolimits_j}}
%% generic open set 
\newcommand{\U}{\mathcal{U}}
%% text referring to the type of document is being compiled
\newcommand{\book}{thesis}
% set
% \newcommand{\bigbrace}[1]{\left\{#1\right\}}
% \newcommand{\set}[2]{\bigbrace{#1\ \left| \ #2 \right.}}
% \newcommand{\setsmall}[2]{\{#1\ | \ #2 \}}

%% j-th interval for continuous time t
\newcommand{\intj}{I^j}
%% J-th interval for continuous time t
\newcommand{\intJ}{I^J}
%% 0-th interval for continuous time t
\newcommand{\intzero}{I^0}
%% shorthand for varepsilon
\newcommand{\eps}{\varepsilon}
%% shorthand for \overline
\newcommand{\ol}[1]{\overline{#1}}
%% shorthand for \underline
\newcommand{\ul}[1]{\underline{#1}}
%% matrix 
\newcommand{\matt}[1]{\begin{bmatrix}#1\end{bmatrix}} 
%% set definition
\newcommand{\bigbrace}[1]{\left\{#1\right\}}
\newcommand{\defset}[2]{\bigbrace{#1\ \left| \ #2 \right.}}
% sign function
\newcommand{\sign}{{\mathop{\rm sign}\nolimits}}
% floor function
\newcommand{\floor}{{\mathop{\rm floor}\nolimits}}
%
\newcommand{\HBC}{hybrid basic conditions}
% vertical vector
\newcommand{\vect}[1]{{\left(\begin{matrix}#1\end{matrix}\right)}}
% CT plants data
%\newcommand{\fp}{\widetilde{f}}


%% LOCALIZATION
\newcommand{\floc}{f_{loc}}
\newcommand{\gloc}{g_{loc}}
\newcommand{\Cloc}{C_{loc}}
\newcommand{\Dloc}{D_{loc}}


%%% UNIFORM FORMULAS FOR STUFF
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% hybrid system with no name and eight parameters:
%% variable, flow set, \in or =, flow map, jump set, \in or =, jump map
\newcommand{\hybridsystem}[7]
{
\left\{
{
\setlength\extrarowheight{.2cm}
\begin{array}{c@{\ }c@{\ }ccc@{\ }c@{\ }c}
#1 &\in&#2 & \ & \dot{#1} & #3 & #4\left(#1\right) \cr
#1 &\in&#5 & \ & {#1}^+   & #6 & #7\left(#1\right)   \cr
\end{array}
}
\right.
}

%% hybrid system with no name and six parameters:
%% variable, flow set, flow map, jump set, jump map
%% inclusions only
\newcommand{\hybridinclusion}[5]
{
\hybridsystem{#1}{#2}{\in}{#3}{#4}{\in}{#5}
}


%% hybrid system with a name and nine parameters:
%% name, variable, flow set, \in or =, flow map, jump set, \in or =, jump map
\newcommand{\hybridsystemwithname}[8]
{
#1: \qquad 
\hybridsystemn{#2}{#3}{#4}{#5}{#6}{#7}{#8}
}


%% hybrid system with a name and seven parameters:
%% name, variable, flow map, flow set, jump map, jump set
\newcommand{\hybridinclusionwithname}[6]
{
#1: \qquad 
\hybridinclusion{#2}{#3}{#4}{#5}{#6}
}

%% hybrid system with logical modes 
%% discrete variable, continuous variable, flow set, \in or =, flow map, jump set, \in or =, jump map (data with no subscripts)
\newcommand{\hybridsystemQ}[8]
{
\left\{
{
\setlength\extrarowheight{.2cm}
\begin{array}{c@{\ }c@{\ }ccc@{\ }c@{\ }c}
#2 & \in & {#3}_{#1} & \ & \dot{#2}    & #4 & {#5}_{#1}\left(#2\right) \cr
#2 & \in & {#6}_{#1} & \ & {(#1,#2)}^+ & #7 & {#8}_{#1}\left(#2\right)  \cr
\end{array}
}
\right.
}


%% data of a hybrid system, first line C, f or F, second line D, g or G. parameters
%% variable, label for C, formula for C, f or F etc, formula for F, label for D, formula for D, g or G etc, formula for G, 
\newcommand{\definehybridsystem}[9]
{
\setlength\extrarowheight{.2cm}
\begin{array}{r@{\ }c@{\ }lcr@{\ }c@{\ }l}
\displaystyle{#2} & = & \displaystyle{#3} & \qquad &
\displaystyle{#4\left(#1\right)} & = & \displaystyle{#5} \\
\displaystyle{#6} & = & \displaystyle{#7} & \qquad &
\displaystyle{#8\left(#1\right)} & = & \displaystyle{#9}
\end{array}
}


%%% Highlight modifications
\def\startmodif{\color{blue}}
\def\stopmodif{\color{black}\normalcolor}



%%% Comments
%\newcommand{\rafal}[1]{{\noindent \color{red} \tt \small #1}}
%\newcommand{\andy}[1]{{\noindent \color{green} \tt \small #1}}
%\newcommand{\ricardo}[1]{{\noindent \color{blue} \tt \small #1}}
%\def\startmodif{\color{red}}
%\def\stopmodif{\color{black}\normalcolor}
%
%\def\startmodifa{\color{green}}
%\def\stopmodifa{\color{black}\normalcolor}
%
%\def\startmodifaa{\color{black}}
%\def\stopmodifaa{\color{black}\normalcolor}
%
%\def\startmodifr{\color{blue}}
%\def\stopmodifr{\color{black}\normalcolor}
%
%\def\startmodifra{\color{black}}
%\def\stopmodifra{\color{black}\normalcolor}


\newcommand{\Sphere}{\mathbb{S}}

\newcommand{\T}{\mathcal{T}}


\newcommand{\diff}{\tiny\mbox{diff}}

\newcommand{\imp}{\tiny\mbox{imp}}













